Two-Stage Session-based Recommendations with Candidate Rank Embeddings

Recent advances in Session-based recommender systems have gained attention due to their potential of providing real-time personalized recommendations with high recall, especially when compared to traditional methods like matrix factorization and item-based collaborative filtering. Nowadays, two of the most recent methods are Short-Term Attention/Memory Priority Model for Session-based Recommendation (STAMP) and Neural Attentive Session-based Recommendation (NARM). However, when these two methods were applied in the similar-item recommendation dataset of Zalando (Fashion-Similar), they did not work out-of-the-box compared to a simple Collaborative-Filtering approach. Aiming for improving the similar-item recommendation, we propose to concentrate efforts on enhancing the rank of the few most relevant items from the original recommendations, by employing the information of the session of the user encoded by an attention network. The efficacy of this strategy was confirmed when using a novel Candidate Rank Embedding that encodes the global ranking information of each candidate in the re-ranking process. Experimental results in Fashion-Similar show significant improvements over the baseline on Recall and MRR at 20, as well as improvements in Click Through Rate based on an online test. Additionally, it is important to point out from the evaluation that was performed the potential of this method on the next click prediction problem because when applied to STAMP and NARM, it improves the Recall and MRR at 20 on two publicly available real-world datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart
OUTPUT_NAME=paper
SAMPLES = \
	$(OUTPUT_NAME).tex \
	$(OUTPUT_NAME)_anonymized.tex \
	$(OUTPUT_NAME)-authordraft.tex \
#	$(OUTPUT_NAME)-xelatex.tex

ROOT_DIR=$(shell pwd)
BUILD_DIR = $(ROOT_DIR)/.build
XELATEX_OPTS=-output-directory=$(BUILD_DIR)

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  directories ${PDF}
	cp $(BUILD_DIR)/*.pdf pdfs/

directories: 
	mkdir -p $(BUILD_DIR) $(ROOT_DIR)/pdfs

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $(XELATEX_OPTS) $<
	pdflatex $(XELATEX_OPTS) $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $(XELATEX_OPTS) $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(BUILD_DIR)/$*.log) \
	do pdflatex $(XELATEX_OPTS) $<; done

%.cls:   %.ins %.dtx
	pdflatex $(XELATEX_OPTS) $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $(XELATEX_OPTS) $<
	cp bibliography.bib $(BUILD_DIR)
	cp ACM-Reference-Format.bst $(BUILD_DIR)
	cd $(BUILD_DIR) && bibtex $*
	pdflatex $(XELATEX_OPTS) $<
	pdflatex $(XELATEX_OPTS) $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(BUILD_DIR)/$*.log) \
	do pdflatex $(XELATEX_OPTS) $<; done

paper-xelatex.pdf:  paper-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $(XELATEX_OPTS) $<
	- bibtex $*
	xelatex $(XELATEX_OPTS) $<
	xelatex $(XELATEX_OPTS) $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(BUILD_DIR)/paper-xelatex.log) \
	do xelatex $(XELATEX_OPTS) $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM) -fr $(BUILD_DIR)/* pdfs/* $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> background.tex <==
% Soften this introduction, explain a bit why encoder-decoder
% maybe something like: recent state-of-the-art models can be dec

%%%%% Jose comments in this section
% * (OPTIONAL) We don't need to explain the encoder-decoder at the beginning. We could explain all the state of the art
% models and at the end talk about encoder of user session and we use E_stamp
% * (OPTIONAL) No need to split i2i in encoder decoder or stmo.
% * "stated in the literature that the next item prediction problem is well-modeled with the encoder-decoder" cite?
% * Instead of using I' use Y_{algorithm_name} to be more clear about what are you referring to. In case of the model
% being a re-ranker you can use Y_{model_name}_{re-ranker}.
% * The same for V as said before.

\section{Background}
The concept of encoder and decoder structure has been widely used in tackling natural language processing
problems \cite{NIPS2014_5346, cho-al-emnlp14, W14-4012},
and has more applications in the recommender system and information retrieval
areas \cite{HidasiKBT15, Li:2017:NAS:3132847.3132926, Sordoni:2015:HRE:2806416.2806493, Li:2017:NAS:3132847.3132926}.
In this section we describe the idea of the encoder-decoder architecture and how the state-of-the-art approaches
we reference can be formulated into this structure.

It has been stated in the literature that the next item prediction problem is well-modeled with the encoder-decoder
architecture.
With this separation, the encoder $E(\cdot)$ focuses on summarizing the user session into a vector representation $h_u$.
The decoder $D(\cdot)$ then takes the session representation $h_u$ and the set of items that can be recommended $Y$ as
input and produce a score $S_Y$ for each item $y \in Y$. Therefore, the recommendation list $L_Y$ is given by:
\begin{equation}
    \label{eq:encoder_decoder}
    \begin{aligned}
        & h_u = E(X_u) \\
        & S_Y = D(h_u, Y) \\
        & L_Y = rank(S_Y)
    \end{aligned}
\end{equation}

The encoder-decoder structure is applicable to not only static methods like Item-Item Collaborative Filtering (I2I-CF),
but also a variety of existing session-based recommenders.
In the following subsections we show how these models can be reformulated as an encoder and a decoder structure.

\subsection{Item-Item Collaborative Filtering (I2I-CF)}
The I2I-CF in non-personalized contexts considers only the most similar items for the last-seen item $x_{l-1}$ in the
user interaction/click sequence.
Each item $x$ in the assortment $I$ is considered as a $\mathbb{R}^{1 \times |U|}$ zero-one vector of user visits,
where $|U|$ denotes the number of users in the dataset.
We reuse the notation $V_x$ for the user visit vector of $x$.

The I2I-CF model can be formulated as an encoder-decoder structure:
\begin{equation}
    \begin{aligned}
        & h_u = E_{I2I}(X_u) = V_{x_{l-1}} \\
        & S_{Y} = D_{I2I}(h_u, Y) = sim(h_u, V_I)
    \end{aligned}
\end{equation}
Where the definition of the similarity function $sim(\cdot)$ is described in \cite{Aiolli2013APS}.

\subsection{Short-Term Memory Only (STMO)}
The STMO model was first mentioned in \cite{Liu:2018:SSA:3219819.3219950} as a baseline recommender,
in which each item is encoded as a feature embedding of shape $\mathbb{R}^{d \times 1}$, and the relationships
between the last item of the sequence and the recommendations are described in a non-linear feed-forward neural network.
The encoder and decoder of this approach are:
\begin{equation}
    \begin{aligned}
        & h_u = E_{STMO}(X_u) = tanh(W^\intercal{V_{x_{l-1}}}) \\
        & S_{Y} = D_{STMO}(h_u, Y) = softmax(h_u^\intercal{V_{Y}})
    \end{aligned}
\end{equation}
Where $W$ is a $\mathbb{R}^{d \times d}$ trainable weight matrix and $V_{Y}$ denotes the vector representation of the
set $Y$, which is of shape $\mathbb{R}^{d \times |Y|}$.
Same as I2I-CF, the STMO model is also a non-personalized model because only the last item $x_{l-1}$ is considered by
the encoder $E_{STMO}$

\subsection{Attention-based GRU (NARM)}
NARM \cite{Li:2017:NAS:3132847.3132926} is one of the state-of-the-art approaches for session-based recommender systems.
For each input user click sequence, the model combines two recurrent neural networks and an attention layer to encode
the user interest and then decode it into a click probability distribution over all the items.
This architecture has a clear definition of encoder and decoder, in this work we use the same definition as
in \cite{Li:2017:NAS:3132847.3132926}.

\subsection{Short-Term Attention Model (STAMP)} \label{stamp_section}
The STAMP model \cite{Liu:2018:SSA:3219819.3219950} is a more light-weight approach compared to NARM, while still
maintaining comparable performance.
It uses attention and feed-forward networks to summarize the user history and encode the whole user session into a
single vector.
The score of an item is then calculated by a three-way inner-product between the session representation, the last
item representation and the embeddings of the items to be ranked.

The STAMP model can also be represented as an encoder-decoder method.
Let $Avg(V_{X_u}) = \frac{1}{l} (\sum_{i=0}^{l-1} V_{x_i})$ be the averaged embedding of the session,
and $ATTN(\cdot)$ the attention operation described in \cite{Liu:2018:SSA:3219819.3219950} in Eq. 7 and Eq. 8.
The encoder and decoder of STAMP can be represented as follows:
\begin{equation}
    \begin{aligned}
        & A_u = ATTN(V_{X_u}, V_{x_{l-1}}, Avg(V_{X_u})) + Avg(V_{X_u})\\
        & h_x = tanh(W_x^\intercal{A_u} + b_x)\\
        & h_a = tanh(W_a^\intercal{V_{x_{l-1}}} + b_a)\\
        & h_u = E_{STAMP}(X_u) = h_x \odot h_a\\
        & S_{Y} = D_{STAMP}(h, Y) = softmax(h_u^\intercal{V_{Y}})
    \end{aligned}
\end{equation}
\begin{figure}
    \includegraphics[height=160pt, width=180pt]{figures/stamp_encoder}
    \caption{The encoder of STAMP model $E_{STAMP}$. In the original paper the authors don't separate their model into
    the encoder and decoder. However, it can still be considered as an encoder-decoder structure.}
    \label{flg:stamp_encoder}
\end{figure}
Where $V_{X_u}$ represents the feature representation of the user history, $\odot$ refers to element-wise product,
and $W_x$, $W_a$, $b_x$, $b_a$ indicate the linear weights and biases of the feed-forward networks.
A graphical illustration of the STAMP encoder is in Figure \ref{flg:stamp_encoder}.

